The Static Center of Pressure Sensitivity: a further Criterion to assess Contact Stability and Balancing Controllers

Legged locomotion has received increasing attention from the robotics community. In this respect, contact stability plays a critical role in ensuring that robots maintain balance, and it is a key element for balancing and walking controllers. The Center of Pressure is a contact stability criterion that defines a point that must be kept strictly inside the support polygon in order to ensure postural stability. In this paper, we introduce the concept of the sensitivity of the static center of pressure: roughly speaking, the rate of change of the center of pressure with respect to the system equilibrium configurations. This new concept can be used as an additional criterion to assess the robustness of the contact stability. We show how the sensitivity of the center of pressure can also be used as a metric to assess balancing controllers by considering two state-of-the-art control strategies. The analytical analysis is performed on a simplified model, and validated during balancing tasks on the iCub humanoid robot.

==> tex/analysis.tex <==
%!TEX root = ../tau_optim.tex
\section{Analysis}
\label{sec:analylis}
\subsection{Contact Forces during a balancing task}

Let's consider the model introduced in the previous section where we have only two external wrenches $f_L$ and $f_R$ resulting from the contact of the robot legs and the ground.
Being a quasi-static scenario, the sum of the external wrenches and the wrench due to gravity must balance, i.e.
\begin{align}
    &W_L + W_R - mg e_2 = 0 \label{eq:momentum_balance} \\
    &W_L = X_L  \prescript{L}{}f_L,\quad  W_R = X_R \prescript{R}{}f_R \notag\\
    & X_L = \begin{bmatrix}
        1_2 & 0_{2\times1} \\ (S\lambda)^\top & 1
    \end{bmatrix},
    X_R = \begin{bmatrix}
        1_2 & 0_{2\times1} \\ (S\rho)^\top & 1
    \end{bmatrix} \notag
\end{align}
where $\lambda$ and $\rho$ are the vectors from the center of mass to the left and right contacts respectively and the left and right wrenches $f_L = \begin{bmatrix}F_L^\top & \mu_L\end{bmatrix}^\top$, $f_R = \begin{bmatrix}F_R^\top & \mu_R\end{bmatrix}^\top$ are composed by the pure forces and pure torques.

Now, we can impose the following form for the contact wrenches:
\begin{equation}
    \label{eq:wrench_decomposition}
    \begin{aligned}
        W_L &= W_m + \Delta \\ 
        W_R &= W_m - \Delta
    \end{aligned}
\end{equation}
The above definition must satisfy \eqref{eq:momentum_balance}. We thus get
\begin{align*}
    W_m &= \frac{W_L + W_R}{2} = \frac{mg}{2}e_2\\
    \Delta &\in \mathbb{R}^3 \quad \text{free} .% \frac{W_L - W_R}{2}\\
\end{align*}
The wrenches expressed at the feet now becomes
\begin{equation}
    \label{eq:wrenches_feet}
    \begin{aligned}
        \prescript{L}{} f_L &= X_L^{-1} W_m + X_L^{-1} \Delta \\
        \prescript{R}{} f_R &= X_R^{-1} W_m - X_R^{-1} \Delta \\
    \end{aligned}    
\end{equation}
By substituting the definition of $W_m$, $X_L$ and of $X_R$ we obtain the following expression:
\begin{equation}
    \label{eq:solution_explicit}
    \begin{aligned}
        \prescript{L}{}f_L &= \frac{mg}{2}\begin{bmatrix}
            0 \\ 1 \\ -\lambda_1
        \end{bmatrix} + X_L^{-1} \Delta \\
        \prescript{R}{}f_R &= \frac{mg}{2}\begin{bmatrix}
            0 \\ 1 \\ -\rho_1
        \end{bmatrix} - X_R^{-1} \Delta
    \end{aligned}
\end{equation}

Because $\Delta$ is a free variable one may be tempted to choose the trivial solution, i.e. $\Delta = 0$.
This choice leads to constant vertical (and equal) forces on both feet, i.e. $(\prescript{L}{}{f_L})_2 = ({\prescript{R}{}{f_R}})_2 = \frac{mg}{2}$. 
They are thus independent of the CoM position.
What, instead, varies with the CoM position are the contact torques which have to compensate for this internal stress.

Notice that the solution obtained with $\Delta = 0$ is similar to the minimum norm solution to \eqref{eq:momentum_balance}.
In fact,
\begin{align*}
    mg e_2 &= W_L + W_R =  
    \begin{bmatrix}
        X_L & X_R
    \end{bmatrix} \begin{bmatrix}
        \prescript{L}{}f_L \\ \prescript{R}{}f_R
    \end{bmatrix} = X f 
\end{align*}

Because, by construction, $X$ is always full row rank we can use the explicit expression of its pseudoinverse to obtain an analytical solution for the wrenches $f$.
In particular, we are interested in the difference between the linear components $\Delta F = F_L - F_R$ which has the following expression:
\begin{equation}
    \label{eq:minimum_norm_solution}
    \begin{aligned}
        \Delta F &= \frac{mg}{4 + \norm{\lambda - \rho}^2} S(\lambda - \rho)(\lambda + \rho)^\top S e_2 \\
        &= - \frac{mg (\lambda_1 - \rho_1)^2}{4 + (\lambda_1 - \rho_1)^2}e_2
    \end{aligned}
\end{equation}
where we used the fact that $\lambda - \rho$ is zero along the $e_2$ axis.

The above equation clearly points out two properties of the solution. 
The first one is that the difference lies only in the vertical component ($e_2$).
The second one is that this difference is function of the distance between the two feet (constant in our scenario), and it is not a function of the CoM position.

This fact is compatible with the analysis performed on the full model of the robot we showed in Section~\ref{sec:background}.
The minimum norm solution of \eqref{eq:momentum_balance} has thus similar effects of the solution \eqref{eq:solution_explicit} with $\Delta = 0$.

% Both the solutions previously obtained may seem counterintuitive, especially while comparing them to what humans do.
% Indeed, one may expect that the force not on the support foot tends to zero as the center of mass moves towards  the support foot.
We now try to find if a different feasible choice of the contact forces leads to a different behaviour.
Let's first consider again \eqref{eq:momentum_balance} but with the forces expressed at the local center of pressure (CoP) instead of the origin of the foot frames.
As a consequence the pure torques are zeros, i.e. \eqref{eq:momentum_balance} rewrites as
\begin{equation*}
    \label{eq:momentum_balance_cop}
    \begin{aligned}
         F_L + F_R & = mg e_2 \\
         \lambda_{cop}^\top S F_L + \rho_{cop}^\top S F_R &= 0
    \end{aligned}
\end{equation*}
where $\lambda_{cop}$ and $\rho_{cop}$ are the vectors connecting the CoM to the center of pressure of the left and right foot respectively. 
Analogously to \eqref{eq:wrench_decomposition} we can decompose the forces as
\begin{equation}
    \label{eq:wrench_decomposition_cop}
    \begin{aligned}
        F_L &= F_m + \tilde{\Delta}\\
        F_R &= F_m - \tilde{\Delta}\\
    \end{aligned}
\end{equation}
where now $\tilde{\Delta} \in \mathbb{R}^2$. By imposing \eqref{eq:momentum_balance_cop}, one obtains
\begin{equation*}
    \begin{aligned}
        F_m &= \frac{mg}{2} e_2 \\
        \tilde{\Delta} &= - \frac{(\lambda_{cop}+\rho_{cop})^\top e_1}{(\lambda_{cop}-\rho_{cop})^\top e_1} \frac{mg}{2}e_2 + \eta e_1
    \end{aligned}
\end{equation*}
with $\eta \in \mathbb{R}$ free.
By substituting the definition of $F_m$ and of $\tilde{\Delta}$ into \eqref{eq:wrench_decomposition_cop} we obtain the final expression for the feet forces:
\begin{equation}
    \label{eq:solution_explicit_cop}
    \begin{aligned}
        F_L &= - \frac{\rho_{cop_1}}{\lambda_{cop_1} - \rho_{cop_1}}mge_2 + \eta e_1 \\
        F_R &=  \frac{\lambda_{cop_1}}{\lambda_{cop_1} - \rho_{cop_1}}mge_2 + \eta e_1
    \end{aligned}
\end{equation}

We can now do the following statement:
\begin{Remark} \label{lemma:cop_forces}
    If $\lambda_{cop_1} \neq \rho_{cop_1} \iff CoP_L \neq CoP_R$ (written w.r.t the world frame) and $\lambda_{cop_1} - \rho_{cop_1}$ is finite, then the vertical right (left) force is equal to zero when the center of mass is above the left (right) center of pressure.
\end{Remark}
\begin{proof}
The proof comes from the application of \eqref{eq:solution_explicit_cop}.
In fact if the CoM is above the left foot, then by definition $\lambda_{cop_1} = 0$. Given \eqref{eq:solution_explicit_cop} and the fact that the denominator is finite by hypothesis then $F_R = 0$. The same reasoning can be applied to the right foot.
The first hypotesis of this remark guarantees that at least one foot must support the weight of the robot.
\end{proof}

\subsection{Choice of the force redundancy}
The analysis conducted in the previous section and the results in Remark~\ref{lemma:cop_forces} shows that the choice of contact forces is responsible of different behaviours in the robot.
A part from the motivations already introduced in Section~\ref{subsec:problem_statement}, forces as in \eqref{eq:solution_explicit_cop} avoid creating internal stress.
We now wonder if there exist a criterion to systematically exploit the redundancy of the forces in \eqref{eq:solution_explicit}, i.e. a choice of the variable $\Delta$, to obtain a behaviour similar to the one stated in Remark~\ref{lemma:cop_forces}.

Because internal stress in the structure is due to internal torques compensating each other, one possible criterion for the choice of $\Delta$ is to use the redundancy to minimize the internal joint torques.
Let's notice however that in case of a mechanical system with heterogeneous joint types, e.g. rotational and prismatic joints, the euclidean norm of the generalized forces is not well defined.
This criterion is anyway justifiable by remembering that the torque produced by an electric motor is proportional to the current absorption and thus to the electric power. Similar considerations can be done for other types of motors.

Assuming rotational joints for simplicity, let's consider \eqref{eq:tau_block_diagonal} and use the wrenches expression in \eqref{eq:wrenches_feet}:
\begin{IEEEeqnarray}{rCl}
    \tau &=& (J_j M_j^{-1})^\dagger J M^{-1} (mge_3 - J_L^\top f_L - J_R^\top f_R) \notag\\
    &=& (J_j M_j^{-1})^\dagger J M^{-1} [ (2 - J_L^\top X_L^{-1} - J_R^\top X_R^{-1}) \frac{mg}{2}e_3 \notag\\
    && - (J_L^\top X_L^{-1} - J_R^\top X_R^{-1}) \Delta] \label{eq:torques_with_delta}
\end{IEEEeqnarray}

By using the definition of the Jacobian of a generic point $p$ as in \eqref{eq:block_diag_relations}
% Recalling the definition of the Jacobian of a generic point $p$ in the dynamical model \eqref{eq:system_dynamics}
% \begin{equation*}
%     J_p^\top =
%     \begin{bmatrix}
%         X_p \\
%         \xoverline{J}^\top_{p,j} - \frac{\xoverline{M}_{bj}^\top}{m} \Lambda^\top X_p
%     \end{bmatrix}
% \end{equation*}
we obtain:
\begin{align*}
    J_L^\top X_L^{-1} + J_R^\top X_R^{-1} &= \begin{bmatrix}
        2~1_6 \\ \xoverline{J}_{L,j}^\top X_L^{-1} + \xoverline{J}_{R,j}^\top X_R^{-1} - 2 \frac{\xoverline{M}_{bj}^\top}{m}\Lambda^\top
    \end{bmatrix} \\
    J_L^\top X_L^{-1} - J_R^\top X_R^{-1} &= \begin{bmatrix}
        0_{6 \times 6} \\
        \xoverline{J}_{L,j}^\top X_L^{-1} - \xoverline{J}_{R,j}^\top X_R^{-1}
    \end{bmatrix}.
\end{align*}

Observe also that 
\begin{equation*}
    P^\top e_3 = \begin{bmatrix}
        0_{3\times 3} & -S(r) \\
        0_{3\times 3} & \frac{I}{m}-1_3
    \end{bmatrix}e_3 = 0_6 \Rightarrow \Lambda^\top e_3 = 1_6
\end{equation*}
then \eqref{eq:torques_with_delta} becomes 
\begin{IEEEeqnarray}{rCl}
    \label{eq:torques_expression_full}
    % \tau &=& (J_j M_j^{-1})^\dagger J \begin{bmatrix} M_b^{-1} & 0 \\ 0 & M_j^{-1} \end{bmatrix}\notag\\
 %    && \left( \right.
 %    \begin{bmatrix}mge_2 - mge_2  \\
 %        -(\xoverline{J}_{jL}^\top X_L^{-1} + \xoverline{J}_{jR}^\top X_R^{-1} - 2 \frac{\xoverline{M}_{bj}^\top}{m})\frac{mg}{2}e_2
 %    \end{bmatrix} \notag\\
 %    &&- \begin{bmatrix}
 %        0_3 \\ \xoverline{J}_{jL}^\top X_L^{-1} - \xoverline{J}_{jR}^\top X_R^{-1}
 %    \end{bmatrix} \Delta \left. \right) \notag\\
   \tau &=& - (J_j M_j^{-1})^\dagger J_j M_j^{-1} \left[\right.(\xoverline{J}_{L,j}^\top X_L^{-1} + \xoverline{J}_{R,j}^\top X_R^{-1} \notag\\
    && - 2 \frac{\xoverline{M}_{bj}^\top}{m})\frac{mg}{2}e_3 + (\xoverline{J}_{L,j}^\top X_L^{-1} - \xoverline{J}_{R,j}^\top X_R^{-1})\Delta\left. \right].
\end{IEEEeqnarray}

When we consider the simplified model, we can notice that if the number of (nonsingular) rows of $J_j$ are greater or equal to the DoFs of the system, as it is in this case, the product of the first two terms yield the identity matrix. 
As a consequence, the vector $\Delta$ which minimizes the joint torques in the four-bar linkage model is given by the solution of
\begin{IEEEeqnarray}{rCl}
    \Delta &=& -\frac{mg}{2} \left(\xoverline{J}_{L,j}^\top X_L^{-1}- \xoverline{J}_{R,j}^\top X_R^{-1}\right)^\dagger \notag \\
    && \left(\xoverline{J}_{L,j}^\top X_L^{-1} + \xoverline{J}_{R,j}^\top X_R^{-1}- 2 \frac{\xoverline{M}_{bj}^\top}{m}\right)e_2 \label{eq:delta_torque_min}
\end{IEEEeqnarray}
which, by using the actual expression for the Jacobians, can be simplified to
\begin{equation}
    \label{eq:delta_simplified_model}
    \Delta = \begin{bmatrix}
        {3 l \cos^2(q_1)}/{10 d \sin(q_1)}\\
        {3l\cos(q_1)}/{10d}\\
        {d}/{4}
    \end{bmatrix}.
\end{equation}

Interestingly, the linear forces are function of $\frac{l}{d}$, i.e. the ratio between the length of the legs and the feet distance. Furthermore, as we expected, they are also function of the angle $q_1$ thus varying with the configuration of the robot.
Figure~\ref{fig:simple_mintorques_forces} shows the vertical forces for the two feet when the choice of $\Delta$ is the one in \eqref{eq:delta_simplified_model}.

\begin{figure}[t]
  \centering
    \includegraphics[width=.9\columnwidth]{imgs/data/simple_mintorques_forces.pdf}
  \caption{Vertical forces for the left and right foot during robot motion for the choice of $\Delta$ as in \eqref{eq:delta_simplified_model}. Forces are normalized by $mg$}
  \label{fig:simple_mintorques_forces}
\end{figure}

\subsection{Analysis of the centers of pressure}
One issue which becomes apparent when applying the obtained wrenches to the system is related to the centers of pressure.
% The choice of $\Delta$ in \eqref{eq:delta_torque_min} is in general not good.
In fact, the CoPs resulting from the forces as in \eqref{eq:wrenches_feet} with $\Delta$ chosen as \eqref{eq:delta_torque_min} tends to infinity.
This is caused by the fact that while the vertical forces goes to zero, their contact moments does not, thus leading to the observed divergence.

An interesting fact is that this property does not strictly depends on the particular criterion to choose $\Delta$.
 % but it is instead related to how  re on the fact that the force goes to zero on the non-support foot and on how its moment is chosen.
To show this fact we can perform an asymptotical analysis on the center of pressure.

Let's recall the definition of the center of pressure, which for the considered 2D case corresponds to a single coordinate along $e_1$:
\begin{equation*}
    CoP = \frac{\mu}{f_{e_2}},
\end{equation*}
which become for two feet:
\begin{equation}
    \label{eq:cop_expression}
    \begin{aligned}
        CoP_L &= \frac{\mu_L}{f_{L_{e_2}}} = \frac{-\frac{1}{2}\lambda_1 + \lambda_2 \Delta_1 - \lambda_1 \Delta_2 + \Delta_3}{\frac{1}{2} + \Delta_2} \\
        CoP_R &= \frac{\mu_R}{f_{R_{e_2}}} = \frac{-\frac{1}{2}\rho_1 - \rho_2 \Delta_1 + \rho_1 \Delta_2 - \Delta_3}{\frac{1}{2} - \Delta_2}.
    \end{aligned}    
\end{equation}

We now focus on the case where the center of mass is on the right foot, i.e. the right foot supports the whole weight. The same consideration can be done equally for the other foot.
Because of this, $f_{R_{e_2}} = mg$, which, as a consequence of \eqref{eq:solution_explicit}, implies $\Delta_2 = -\frac{1}{2}$.
The CoP of the left foot thus become
\begin{align*}
    CoP_L &= \lim_{\Delta_2 \rightarrow -\frac{1}{2}} \frac{-\frac{1}{2}\lambda_1 + \lambda_2 \Delta_1 - \lambda_1 \Delta_2 + \Delta_3}{\frac{1}{2} + \Delta_2} \\
    &= \frac{\lambda_2 \Delta_1 + \Delta_3}{0}.
\end{align*}

The result of the above expression depends on the value of the numerator, i.e. of $\lambda_2 \Delta_1 + \Delta_3$.
Indeed, if it is different from zero, then the CoP tends to $\pm \infty$.
If, instead, it goes to zero faster then the denominator, the CoP tends to zero.

If we consider the expression of $\Delta$ in \eqref{eq:delta_simplified_model} we can verify that the CoP diverges. 
In fact
\begin{align*}
    &\Delta_2 = -\frac{1}{2} \Rightarrow \cos(q_1) = - \frac{5d}{3l} \\
    &\Rightarrow \Delta_1 = \frac{5d}{6l\sin(q_1)}, \quad \Delta_3 = \frac{d}{4}.
\end{align*}
Furthermore $\lambda_2$ has the following expression:
\begin{equation*}
    \lambda_2 = %\frac{2m_B + m_L + m_R}{m_B + m_L + m_R} \frac{l}{4} \sin(q_1) 
     -\alpha \frac{l}{2} \sin(q_1) 
\end{equation*}
where $\alpha > 1$ is a term which depends on the mass of the three rods. By plugging everything together we get:
\begin{align*}
    \lambda_2 \Delta_1 + \Delta_3 &= -\alpha \frac{l}{2} \sin(q_1)  \frac{5d}{6l\sin(q_1)} + \frac{d}{4} = \frac{d(3 - 5 \alpha)}{12} < 0.
\end{align*}
Given the above result $CoP_L \rightarrow - \infty$.

\begin{figure}[t]
  \centering
    \includegraphics[width=.9\columnwidth]{imgs/data/simple_mintorques_cop.pdf}
  \caption{Left and right foot CoPs, and CoM during robot motion. The asymptot is in  correspondence of the forces going to zero}
  \label{fig:simple_mintorques_cop}
\end{figure}

Figure~\ref{fig:simple_mintorques_cop} shows the CoPs during the robot motion. Notice that the CoP of the left foot goes to $-\infty$ when the left force in Figure~\ref{fig:simple_mintorques_forces} goes to zero, as expected.

It is interesting to compare the obtained CoPs and wrenches with the results from Remark~\ref{lemma:cop_forces}.
The hypothesis of the statement in this case are not satisfied.
When the center of mass is on top of one CoP, the two CoP coincides, i.e. $\lambda_{cop_1} - \rho_{cop_1} = 0$. 
% If we consider the point where the vertical force goes to zero, then it is the CoPs which goes to infinity.

Different solutions can be put into effect in order to satisfy Remark~\ref{lemma:cop_forces} and thus having limited CoPs while forces go to zero.
One possible way is to find a new optimization criterion to exploit the forces redundancy.
Alternatively, one can try to impose conditions on the first and third components of $\Delta$ in \eqref{eq:cop_expression}.
Indeed, trying to impose that the numerator goes to zero faster than the denominator can result in a nonlinear problem.

A pragmatic approach, instead, is to use a QP solver to include inequalities on the CoPs. Note that in a real world application, inequalities are anyways needed to satisfy friction cones, joint torque limits, and other constraints.

\begin{figure}[t]
  \centering
    \includegraphics[width=.9\columnwidth]{imgs/data/simple_mintorques_qp_cop.pdf}
  \caption{Left and right foot CoPs, and CoM during robot motion. CoPs remains limited because of the presence of the QP solver}
  \label{fig:simple_mintorques_qp_cop}
\end{figure}

If we solve \eqref{eq:torques_expression_full} by using a dedicated solver we obtain the CoPs as in Figure~\ref{fig:simple_mintorques_qp_cop}. 
Forces are not shown because they are similar to the ones in Figure~\ref{fig:simple_mintorques_forces}. 
We can note that in this case the center of mass is on top of the center of pressure when the force goes to zero, both for the left foot and for the right foot. The hypotesis of Remark~\ref{lemma:cop_forces} are indeed satisfied.

\subsection{Static CoP Sensitivity Analysis}

We now analyse the sensitivity of the static CoP for the four-bar linkage model when we apply the two different forces solution in \eqref{} and \eqref{eq:torques_expression_full}.
We show the analysis we performed on the right foot, but the same results can be drawn for the left foot.

If we denote with $q$ the minimum coordinate of the constrained four-bar linkage model we can differentiate the CoP expression, that is
\begin{align*}
    \frac{\partial CoP_R}{\partial q} &= \frac{\partial}{\partial q} \left(\frac{12 l \cos(q)}{5 d^2 - 6 l d \cos(q) + 20}\right) \\
    & = -60 l \sin(q) \frac{d^2 + 4}{(5 d^2 - 6 l d \cos(q) + 20)^2}
\end{align*}

If, instead, we use the forces in \eqref{} we obtain the following expression for the static CoP sensitivity
\begin{align*}
   \frac{\partial CoP_R}{\partial q} &= \frac{\partial}{\partial q} \left(\frac{3ld\cos(q)}{10d - 6l\cos(q)} \right) \\
   & = - \frac{15 l d^2 \sin(q)}{2(5d - 3l\cos(q))^2}
\end{align*}

\begin{figure}[t]
  \centering
    \includegraphics[width=.9\columnwidth]{imgs/data/simple_all_cop.pdf}
  \caption{Comparison between the right foot CoPs for two different forces choice. The CoM is also plotted in yellow}
  \label{fig:simple_all_cop}
\end{figure}

Figure \ref{fig:simple_all_cop} shows the numerical simulations of the CoP of the right foot.
If we compute the sensitivity at the initial configuration, i.e. $q = \frac{\pi}{2}$, and we use $d = 0.2 \mathrm{m}$ and $l = 1 \mathrm{m}$ we obtain the following values for the two solutions: $-0.5941 \mathrm{m/rad}$ and $-0.3 \mathrm{m/rad}$, i.e. the minimum torque solution is twice less sensitive than the minimum force norm solution.




==> tex/diag.tex <==
%!TEX root = ../tau_optim.tex
\section{Average velocity decouples \\ joint and base frame accelerations }
\label{sec:decoupling}
Prior to applying the above results  to a specific robot model, this section presents a new expression of the  equations of motion~\eqref{eq:system_dynamics}. In particular, the next lemma presents a change of coordinates in the state space $(q,\xoverline{\nu})$ that transforms the system dynamics~\eqref{eq:system_dynamics} into a new form where the mass matrix is block diagonal, thus decoupling joint and base frame accelerations. The obtained equations of motion are then used in 
Section~\ref{sec:four-bar}.

\vspace{0.5cm}
\begin{boldLemma}
\label{lemma:silvioTranfs}
Consider the equations of motion given by~\eqref{eq:system_dynamics}. Perform the following  change of state variables:
\begin{align}
q := {q}, ~~ \nu := T(q)\xoverline{\nu}, \IEEEyessubnumber
\label{eq:centroidalTransform}
\end{align}
with 
\begin{align}
T &:= \begin{bmatrix}
        \prescript{c}{}X_{b} & T_s \\
        0_{n \times 6} & 1_n
    \end{bmatrix}, \\
    T_s &:= \prescript{c}{}X_{b} \xoverline{M}^{-1}_b \xoverline{M}_{bj} \\
    \prescript{c}{}X_{b} &:= \begin{bmatrix}
        1_3 & -S(\prescript{\mathcal{I}}{}p_{c}-\prescript{\mathcal{I}}{}p_{\mathcal{B}}) \\ 
        0_{3 \times 3} & 1_3
    \end{bmatrix}.
\end{align}
Then, the equations of motion with state variables $(q,\nu)$ can be written in the following form
%assume a form in which the derivative of the first six elements of $\nu$ are independent etc etc TO COMPLETE, i.e. : 
\begin{align}
    \label{eq:decoupled_system_dynamics}
    M(q)\dot{\nu} + C(q, \nu) \nu + G = B \tau + \sum_{k = 1}^{n_c} J^\top_{\mathcal{C}_k} f_k,
\end{align}
with
\begin{subequations}
\begin{align}
   \label{eq:massMatrixStructure}
    M(q) &= T^{-\top} \xoverline{M} T^{-1} = \begin{bmatrix}
        M_b(q) & 0_{6\times n} \\ 0_{n\times 6} & M_j(q_j)
    \end{bmatrix},
\end{align}
\begin{align}
    \label{eq:coriolisMatrixStructure}
    C(q,\nu) &= T^{-\top}(\xoverline{M}\dot{T}^{-1} + \xoverline{C}T^{-1}) \notag\\
    & = 
    \begin{bmatrix}
    0_{3\times3} & 0_{3\times3} & 0_{3\times n} \\
    0_{3\times3} & C_b(q,\nu)   & C_{bj}(q,\nu)     \\
    0_{3\times3} & -C_{bj}^\top(q,\nu)  & C_j(q,\nu)  \\ 
    \end{bmatrix},
\end{align}
\begin{align}
   \label{eq:gravityStructure}
    G &= T^{-\top}\xoverline{G} = mge_3,
\end{align}
\begin{align}
    \label{eq:jacobianStructure}
     J_{\mathcal{C}_k}(q) = \xoverline{J}_{\mathcal{C}_k}(q) T^{-1} = \begin{bmatrix} J_{\mathcal{C}_k}^b(q) & J_{\mathcal{C}_k}^j(q_j)\end{bmatrix},
 \end{align}
 \begin{align*}
    M_b(q) &= \begin{bmatrix}
        m 1_3 & 0_{3\times3} \\ 0_{3\times3} & I(q)
    \end{bmatrix}, ~
 J_{\mathcal{C}_k}^b(q) =
 \begin{bmatrix}
 1_3 & {-}S(\prescript{\mathcal{I}}{}p_{\mathcal{C}_k}{-}\prescript{\mathcal{I}}{}p_{c})  \\ 
 0_{3\times3} & 1_3 \\ 
 \end{bmatrix}
 \end{align*}
 %\begin{align*}
 %\Lambda &= 1_6 - P (1_6 + \prescript{c}{}X_b^{-1} P)^{-1} \prescript{c}{}X_b^{-1} \\
 %P &= \begin{bmatrix}
 %    0_{3\times 3} & 0_{3\times 3} \\ S(\prescript{\mathcal{I}}{}p_{c}-\prescript{\mathcal{I}}{}p_{\mathcal{B}}) & \frac{I}{m} - 1_3
 % \end{bmatrix}
%\end{align*}
\end{subequations}
\end{boldLemma}

The above lemma points out that the mass matrix of the transformed system~\eqref{eq:decoupled_system_dynamics} is block diagonal, i.e. the transformed base acceleration is independent from the joint acceleration. More precisely, 
%First, let us observe that 
the transformed robot's velocity $\nu$ is given by  
\begin{IEEEeqnarray}{RCL}
\label{eq:newNu}
\nu &=& 
\begin{pmatrix}
^\mathcal{I}\dot{p}_c \\
^\mathcal{I}\omega_c \\
\dot{q}_j
\end{pmatrix} 
\end{IEEEeqnarray}
where $^\mathcal{I}\dot{p}_c$ is the velocity of the center-of-mass of the robot, and
$^\mathcal{I}\omega_c$ is the so-called \emph{average angular velocity}\footnote{The term $^\mathcal{I}\dot{\omega}_c$ is also known as the \emph{locked angular velocity}~\cite{marsden1993reduced}.}\cite{jellinek1989separation,essen1993average,orin2013}.
% In fact, it is possible to verify that the angular velocity $^\mathcal{I}\omega_c$ coincides with the \emph{average angular velocity} of the multi-body system introduced in~\cite{orin2013}.
% with respect to the inertial frame. 
% Then, the acceleration $(^\mathcal{I}\ddot{p}_c,
%^\mathcal{I}\dot{\omega}_c)$ is independent from the joint acceleration $\ddot{q}_j$. 
Hence,
Eq.~\eqref{eq:decoupled_system_dynamics} unifies what the specialized robotic literature usually presents with two sets of equations: the equations of motion of the free floating system and the \emph{centroidal dynamics}\footnote{In the specialized literature, the terms \emph{centroidal dynamics} are used  to indicate the rate of change of the robot's momentum expressed at the center-of-mass, which then equals to the summation of all external wrenches acting on the multi-body system \cite{orin2013}.}  when expressed in terms of the \emph{average angular velocity}. For the sake of correctness, let us remark that defining the \emph{average angular velocity} as the angular velocity of the multi-body system is not theoretically sound. In fact, the existence of a rotation matrix $R(q)\in SO(3)$ such that  $\dot{R}(q)R^\top(q) = S(^\mathcal{I}\omega_c)$, i.e. the integrability of $^\mathcal{I}\omega_c$,  is still an open issue.
  
Observe also that the Coriolis term $C(q,\nu)$ is \emph{quasi} block diagonal, and that the gravity term $G$ is constant and influences the acceleration of the center-of-mass only.
%The joint torques are not instantaneously related to the com acceleration and the angular acceleration.
 
%\begin{equation}
%m ^\mathcal{I}\ddot{p}_c = 
% \sum_{k = 1}^{n_c} 
% \begin{bmatrix}
%1_3 & 0_{3\times3} 
%\end{bmatrix}
% f_k + mge_3
%\end{equation}

%$^\mathcal{I}\omega_C$ is known in literature as the \emph{average angular velocity} \cite{jellinek1989separation,essen1993average,orin2013} or \emph{locked angular velocity} \cite{marsden1993reduced} of the multibody system.
% Despite its name, it is not defined as the angular velocity of any physical frame. In this paper we define it simply as the result of the transformation \eqref{eq:centroidalTransform}, without any assumption on its nature. 

A transformation similar to~\eqref{eq:centroidalTransform} was presented in  \cite{garofalo2015inertially}. The transformation in this work, however, is from the state 
$(q,\xoverline{\nu})$ into a mixed state, which is composed of the robot's momentum and velocity. Thus it does not represent classical transformations of the state space.
%, in which the linear and angular momentum are used in the transformed state in place of the COM velocity and the locked angular velocity. The main advantage of the proposed approach is that the resulting contact Jacobian (in particular the first six columns of it) are quite simpler. 

==> tex/fourbar_copy.tex <==
%!TEX root = ../tau_optim.tex
% \section{On the effects of minimizing joint torques: \\ the case study of the four-bar linkage}
\section{Analysis and results on a simplified system:\\ the four-bar linkage model}
\label{sec:four-bar}
This section studies how the sensitivity of the static center of pressure introduced in the previous section differs depending on the choice of the contact wrenches.
We decide to perform the analytical analysis on a four-bar linkage when standing on two, flat, rigid contacts. 
As the experimental results in Section~\ref{sec:experiments} show, the chosen case study  is representative of a humanoid robot standing on two feet.
More precisely
what follows shows that minimizing the joint torques when the Newton-Euler equations are at the equilibrium can bring benefits in terms of the \emph{static center of pressure sensitivity}, thus improving the stability of the contact.
% This section studies the effects of minimizing joint torques of a four-bar linkage when standing on two, flat, rigid contacts.
% As the experimental results in Section~\ref{sec:experiments} show, the chosen case study  is representative of a humanoid robot standing on two feet.
% More precisely
% % , by using the contributions in Sections~\ref{sec:scop} and~\ref{sec:decoupling},
% what follows shows that minimizing the joint torques when the Newton-Euler equations are at the equilibrium can bring benefits in terms of the \emph{static center of pressure sensitivity}, thus improving the stability of the contact.
\subsection{Modelling}
\begin{figure}[t]
    \centering{
    % \includsvg{imgs/model}
        \def\svgwidth{\columnwidth}
        \input{imgs/model.pdf_tex}
    \caption{Free floating planar four-bar linkage}
    \label{fig:simple_model}
    }
\end{figure}

Consider the  four-bar linkage shown in Figure~\ref{fig:simple_model}, where $l$ and 
$d$ denote the lengths of the leg and of the upper rod, respectively.
The inertial frame $\mathcal{I}$ is chosen so as the $y$ axis opposes gravity, the $z$ axis exits from the plane, and the $x$ axis completes the right-hand base.
Being a planar model,  only translations in the $x-y$ plane and rotations about the $z$ axis are allowed. Let $^\mathcal{I}{p}_\mathcal{B} \in \mathbb{R}^2$ denote the position of the origin of the frame~$\mathcal{B}$ --which is located at the center of the upper rod-- expressed in the inertial frame. The configuration space is then parametrized by the following coordinates 
\[q = (^\mathcal{I}{p}_\mathcal{B},\theta, q_1,q_2,q_3,q_4) \in \mathbb{R}^7.\]
Being a vector space, to derive the equations of motion, we use the Lagrange formalism with the assumption that any link composing the four-bar linkage can be approximated as a point-mass located at the center of the link. 
In addition, we also assume that the mass of the left leg equals the mass of the right leg. % Hence, let $\mathcal{L} = \mathcal{T} - \mathcal{U}$ denote the \emph{Lagrangian}, with $\mathcal{T}$ and $\mathcal{U}$ the kinetic and potential energies of the system, respectively. 
% The equations of motion in the form~\eqref{eq:system_dynamics} are thus given by 
% \begin{IEEEeqnarray}{RCL}
% 	\frac{d}{dt}\frac{\partial}{\partial \dot{q}} \mathcal{L} 
%	- \frac{\partial}{\partial q} \mathcal{L} &=& 
%	\begin{pmatrix}
%	0_{3\times 1} \\
%	\tau
%	\end{pmatrix}.
% \end{IEEEeqnarray}
Due to the lack of space, the complete dynamic model is not presented here. 
We present only the terms of the dynamic and kinematic model that are necessary to the remainder of the section. In particular, partition the mass matrix $\xoverline{M}$ as follows 
\begin{IEEEeqnarray}{RCL}
\xoverline{M} &=& 
\begin{bmatrix}
	\xoverline{M}_b && \xoverline{M}_{bj} \\
	\xoverline{M}^\top_{bj} && \xoverline{M}_{j}
\end{bmatrix}.
\nonumber
\end{IEEEeqnarray}
Let $\sin(q_i) = s_i$ and $\cos(q_i) = c_i$. One can verify that 
\begin{IEEEeqnarray}{RCL}
\label{MbjFourBarLink}
\xoverline{M}_{bj} &=& \frac{m_l}{2}
\begin{bmatrix}
	l s_1 & 0 & l s_3 & 0 \\
	- l c_1 & 0 & - l c_3 & 0 \\
	 \frac{l^2 s^2_1 {-} l c_1(d{-}l c1)}{2} & 0 &  \frac{l^2 s^2_3 {+} l c_3(d{+}l c_3)}{2} & 0 
\end{bmatrix} \IEEEeqnarraynumspace
\end{IEEEeqnarray}
where $m_l$ is the mass of either leg.
The feet Jacobians are given by the following expression
\begin{equation*}
    \label{eq:fourbarJacobian}
    \begin{aligned}
        \xoverline{J}_{\mathcal{C}_L} &=
        \left[\begin{array}{c c c c c c c}
             &  &  &  & 0 & 0 & 0 \\
            \multicolumn{2}{c}{\smash{\raisebox{.5\normalbaselineskip}{$1_2$}}} &
            \smash{\raisebox{.5\normalbaselineskip}{$R(\theta)\begin{bmatrix}
                ls_1\\ \frac{d}{2} -l c_1
            \end{bmatrix}$}} 
            & \smash{\raisebox{.5\normalbaselineskip}{$R(\theta)\begin{bmatrix}
                l  s_1\\
                -l  c_1
            \end{bmatrix}$}} & 0 & 0 & 0 \\
            % [-\normalbaselineskip]
            0 & 0 & 1 & 1 & 1 & 0 & 0
        \end{array}\right]\\
        \xoverline{J}_{\mathcal{C}_R} &=
        \left[\begin{array}{c c c c c c c}
             &  &  &   0 & 0 & & 0 \\
            \multicolumn{2}{c}{\smash{\raisebox{.5\normalbaselineskip}{$1_2$}}} &
            \smash{\raisebox{.5\normalbaselineskip}{$R(\theta) \begin{bmatrix}
                ls_3\\ -\frac{d}{2} +l c_3
            \end{bmatrix}$}} 
            & 0 & 0 & \smash{\raisebox{.5\normalbaselineskip}{$R(\theta) \begin{bmatrix}
                l s_3 \\ -l c_3
            \end{bmatrix}$}}  & 0 \\
            % [-\normalbaselineskip]
            0 & 0 & 1 & 0 & 0 & 1 & 1
        \end{array}\right].
    \end{aligned}
\end{equation*}



To represent a classical balancing context of humanoid robots, we assume that the mechanism makes contact with the environment at the two extremities. Also, we assume  that 
the distance between the contacts equals the length $d$ of the upper rod -- see Figure \ref{fig:fourBarLinkageStanding}. Then, the rigid constraint acting on the system takes the form~\eqref{eqn:completeConstraintAcc}, with 
$\xoverline{J} = 
\begin{bmatrix}
\xoverline{J}_{\mathcal{C}_L}^\top  &
\xoverline{J}_{\mathcal{C}_R}^\top
\end{bmatrix}^\top \in \mathbb{R}^{6 \times 7}
$,
and
$\nu = \dot{q}$. The associated contact wrenches are $f = (f_L,f_R) \in \mathbb{R}^6$.
As a consequence of these constraints, the mechanism  possesses one degree of freedom when standing on the extremities.

With the aim of evaluating the sensitivity of the static center of pressure, observe that
the mapping $\chi(\xi)$ in~\eqref{eqn:mappinMinimulCoorConfSpa} is given by:
\begin{IEEEeqnarray}{RCL}
\begin{bmatrix}
^\mathcal{I}{p}_b \\
\theta \\ 
 q_1 \\
 q_2 \\ 
 q_3 \\
 q_4 \\
\end{bmatrix} &=&
\begin{bmatrix}
\tfrac{1}{2}d e_1 + l \sin(\xi) e_2+ l \cos(\xi) e_1 \\
0 \\ 
 \xi \\
\pi -\xi \\ 
 \xi \\
 \pi-\xi \\
\end{bmatrix}.
\end{IEEEeqnarray}

\subsection{Choice of the contact forces}

Remark that in order to evaluate the sensitivity of the static center of pressure, we need an expression for the contact forces at the equilibrium configuration -- see Definition~\ref{def:scopSens}.
What follows proposes an analysis of the sensitivity of the static center of pressures evaluated with contact wrenches obtained from two criteria.
\begin{enumerate}
\item The contact wrenches ensure the equilibrium of the centroidal dynamics written in the plane --~i.e. three equations.   
The three dimensional redundancy of the contact wrenches minimize the norm of the contact wrenches $|f|$ \footnote{It is worth noting that the norm of a wrench is not well defined and highly dependent on the metric chosen. Nevertheless, the minimisation of the contact wrench norm is something extensively done in literature and it has been used in the manuscript only for comparison purposes.}.
\item The contact wrenches ensure the equilibrium of the centroidal dynamics.
The three dimensional redundancy of the contact wrenches minimize the norm of the joint torques $|\tau|$.
\end{enumerate}

More precisely, being the balance of the external wrenches acting on the mechanism, the centroidal dynamics is simply given by 
\begin{align}
    \label{eq:momentum_balance}
     0 & = X_L \prescript{L}{}f_L + X_R \prescript{R}{}f_R - m g e_2 = X f - mge_2
\end{align}
where $mge_2$ is the wrench due to gravity and $X := \begin{bmatrix}
    X_L & X_R
\end{bmatrix}$,
\begin{equation*}
    X_L = \begin{bmatrix}
            1_2 & 0_{2\times1} \\ (S\lambda)^\top & 1
        \end{bmatrix},
        X_R = \begin{bmatrix}
            1_2 & 0_{2\times1} \\ (S\rho)^\top & 1
        \end{bmatrix},
\end{equation*}
 $\lambda = \begin{bmatrix}
    \lambda_1 & \lambda_2
\end{bmatrix}^\top \in \mathbb{R}^2$ and $\rho = \begin{bmatrix}
    \rho_1 & \rho_2
\end{bmatrix}^\top \in \mathbb{R}^2$ the vectors connecting the center of mass to the left and right feet frames respectively. 

Since $X \in \mathbb{R}^{3 \times 6}$ is always full row rank by construction, \eqref{eq:momentum_balance} admits infinite solutions, i.e.
\begin{equation}
    \label{eq:4bar_minforces}
    f = X^\dagger
    % \begin{bmatrix}
    %     \prescript{L}{}f_L\\
    %     \prescript{R}{}f_R
    % \end{bmatrix}
    %  = \begin{bmatrix}
    %      X_L & X_R
    %  \end{bmatrix}^\dagger
      mge_2 + N_f f_0
\end{equation}
where $X^\dagger \in \mathbb{R}^{6\times3}$ is the Moore-Penrose pseudoinverse of $X$, $N_f \in \mathbb{R}^{6\times6}$ is the projector onto the nullspace of $X$ and $f_0 \in \mathbb{R}^6$ is a free variable.

Then, the criterion $1)$ corresponds to the choice $f_0 = 0$. The criterion $2)$, instead, involves the evaluation of the joint torques associated with the wrenches $f$, and then the exploitation of $f_0$ to minimize the joint torques.

\subsubsection{Minimum contact wrench norm solution}
By setting $f_0 = 0$ in Eq.~\eqref{eq:4bar_minforces}, one can show that 
 the wrench acting on the right foot is given by
\begin{equation*}
    \prescript{R}{}f_R =
    \frac{1}{mg}
    \begin{bmatrix}
         0\\[0.5em]
         \frac{20 + 5 d^2 + 6ld \cos(\xi)}{10 (d^2 + 4)} \\[0.5em]
         \frac{6ld \cos(\xi)}{5 (d^2 + 4)}
    \end{bmatrix}.
\end{equation*}
If $d$ is small, e.g. the distance between the two feet is smaller than one meter, then the above expression points out that one has an \emph{almost} constant vertical force --~approximately equal to $mg/2$~-- independently of $\xi$, i.e. independently of the center-of-mass position.

Figure~\ref{fig:simple_minforces_cop} shows the static CoP of the left and right foot in correspondence of the CoM motion. We can notice how $\sigma_L$ and $\sigma_R$ moves together with the CoM leading to the breakage of the contact.

\begin{figure}[t]
  \centering
    \includegraphics[width=.9\columnwidth]{imgs/data/simple_minforces_cop.pdf}
  \caption{Left and right foot CoPs for the minimum wrenches norm solution. The CoM is plotted in yellow}
  \label{fig:simple_minforces_cop}
\end{figure}

To evaluate the static center of pressure sensitivity, we can differentiate the CoP expression w.r.t $\xi$, that is
\begin{align*}
   \eta_R &= \frac{\partial \sigma_R}{\partial \xi} = \frac{\partial}{\partial \xi} \left(\frac{12 l \cos(\xi)}{5 d^2 - 6 l d \cos(\xi) + 20}\right) \\
    & = -60 l \sin(\xi) \frac{d^2 + 4}{(5 d^2 - 6 l d \cos(\xi) + 20)^2}.
\end{align*}

\begin{corollary}
    The solution which exploits the force redundancy to minimize the tangential component of the contact wrenches is equivalent to the minimum contact wrenches norm solution.
\end{corollary}
\begin{proof}
    Consider Eq. \eqref{eq:4bar_minforces}. We want to use $f_0$ to minimize the tangential component of the contact wrenches, i.e. we want find the solution to
    \begin{equation*}
        \begin{bmatrix}
            e_1^\top \\
            e_4^\top 
        \end{bmatrix} f = 0 \iff \begin{bmatrix}
            e_1^\top \\
            e_4^\top 
        \end{bmatrix} N_f f_0 + \begin{bmatrix}
            e_1^\top \\
            e_4^\top 
        \end{bmatrix} X^\dagger mge_2 = 0.
    \end{equation*}
    Because of the expression of the nullspace projector and of the pseudoinverse, the above equation reduces to
    \begin{equation*}
        \frac{1}{2}
        \begin{bmatrix}
            1 & 0 & 0 & -1 & 0 & 0 \\
            -1 & 0 & 0 &  1 & 0 & 0
        \end{bmatrix} f_0 = 0
    \end{equation*}
    which has the minimum norm solution in $f_0 = 0$.
\end{proof}

\subsubsection{Minimum joint torque norm solution}

Consider again the balance of the external wrenches acting on an articulated rigid body in the general $3$D case:
\begin{align}
        \label{eq:momentum_balance3D}
      X_L \prescript{L}{}f_L + X_R \prescript{R}{}f_R - m g e_3 = 0
\end{align}
where $X_L,X_R \in \mathbb{R}^{6\times6}$ are used to express the wrenches respectively in $L$ and $R$ at the center of mass.
Impose the following expression for the contact wrenches:
\begin{equation}
    \label{eq:wrenches_feet}
    \begin{aligned}
        \prescript{L}{} f_L &= X_L^{-1} \frac{mg}{2}e_3 + X_L^{-1} \Delta \\
        \prescript{R}{} f_R &= X_R^{-1} \frac{mg}{2}e_3 - X_R^{-1} \Delta
    \end{aligned}  
\end{equation}
where $\Delta \in \mathbb{R}^6$ is a free variable.
We can notice that with the above choice, \eqref{eq:momentum_balance3D} is always satisfied independently of the choice of $\Delta$.
In what follows, the redundancy $\Delta$ is used to minimize the joint torques.
To simplify the calculations we perform a state transformation as described in \cite{Traversaro2016}.
In particular, the dynamics in the new state variables is decoupled in the acceleration, i.e. the mass matrix is block diagonal, with the two blocks being the terms relative to the base and the joints.
We refer the reader to \cite{Traversaro2016} for additional details, and we report here only the relevant transformations.
To avoid confusion, all the dynamic quantities in the new state variables are denoted without the overline. 

The new base frame is chosen to correspond to a frame with the same orientation of the inertial frame $\mathcal{I}$ and the origin instantaneously located at the center of mass.
We denote with ${}^c X_\mathcal{B}$
% \[
%     {}^c X_\mathcal{B} = \begin{bmatrix}
%         1_3 & S()\\
%         0_{3 \times 3} & 1_3
%     \end{bmatrix}
% \]
 the corresponding $6$D transformation.
% The new acceleration-decoupled dynamic equations are then denoted without the bar.
Of particular interest is the form of the Jacobian of the left (right) foot frame $L$ ($R$) in the new state variables:
\begin{align}
    \label{eq:jacobian_new}
    J_{{L}} &= \begin{bmatrix}
        J_{{L}}^b & J_{{L}}^j
    \end{bmatrix} = \begin{bmatrix}
        X_{{L}}^\top & \xoverline{J}_{{L}}^j - \frac{1}{m}X_{{L}}^\top \Lambda \xoverline{M}_{bj}
    \end{bmatrix}, \\
    \Lambda &:=  1_6  - P ( 1_6 + {}^c X_B^{-1} P)^{-1}{}^cX^{-1}_B \notag
\end{align}
with $P$ the following matrix:
\begin{equation*}
    P := \begin{bmatrix}
        0_{3\times3} & 0_{3\times3} \\
        S(p_{\text{CoM}} - p_\mathcal{B}) & \frac{I}{m} - 1_3 
    \end{bmatrix}
\end{equation*}
where $I$ is the $3$D inertia of the robot expressed w.r.t. the orientation of $\mathcal{I}$ and the center of mass as origin and $p_{\text{CoM}} - p_\mathcal{B}$ is the distance between the center of mass and the base frame before the state transformation.
%We would like to find a criterion to automatically choose the free variable $\Delta$ while obtaining some benefits w.r.t. the trivial choice of $f_0 = 0$. 
%One possible option is to determine $\Delta$ such that the resulting internal torques are minimized.
%Let's notice however that in case of a mechanical system with heterogeneous joint types, e.g. rotational and prismatic joints, the euclidean norm of the generalized forces is not well defined.
%This criterion is anyway justifiable by remembering that the torque produced by an electric motor is proportional to the current absorption and thus to the electric power. Similar considerations can be done for other types of motors.

The relation between the joint torques and the contact wrenches is given by Eq.~\eqref{eq:contactforcesEq}. So, by inverting this relation, we evaluate the effects of the contact wrench redundancy $\Delta$ on the joint torques at the equilibrium configuration, i.e.
%We start by considering the dynamical system \eqref{eq:decoupled_system_dynamics} subject to rigid constrains as in \eqref{eqn:completeConstraintAcc}. 
%By constraining the system we obtain the following expression:
%\begin{equation}
%    \label{eq:tau_expression}
%   JM^{-1}B \tau = JM^{-1}(C \nu + g - J^\top f) - \dot{J} \nu.
%\end{equation}
%We can now describe the solution set, i.e. obtain the function $\tau = \tau(f, \tau_0)$ by solving it for $\tau$:
%\begin{equation}
%   \label{eq:tau_generic}
%   \tau = (J M^{-1}B)^\dagger [JM^{-1} (C \nu + g  - J^\top f) - \dot{J} \nu] + N_\tau \tau_0
%\end{equation}
%where $N_\tau$ is a projector onto the nullspace of $(J M^{-1}B)$ and $\tau_0$ is the associated free variable.
%
%If we now impose the static condition, i.e. $\nu = 0$, and the fact that \eqref{eq:decoupled_system_dynamics} is decoupled in the accelerations, one obtains
\begin{equation}
    \label{eq:tau_general_system}
    \tau = (J_j M_j^{-1})^\dagger J M^{-1} (mge_3 - J^\top f).
\end{equation}
%where we set $\tau_0 = 0$.
We can now substitute the definition of $f$ as in \eqref{eq:wrenches_feet} into the obtained expression of $\tau = \tau(f)$ in \eqref{eq:tau_general_system}, i.e. 
\begin{IEEEeqnarray}{rCl}
    \tau &=& 
    %(J_j M_j^{-1})^\dagger J M^{-1} (mge_3 - J_L^\top f_L - J_R^\top f_R) \notag\\
%    &=&
     (J_j M_j^{-1})^\dagger J M^{-1} [ (2 - J_L^\top X_L^{-1} - J_R^\top X_R^{-1}) \frac{mg}{2}e_3 \notag\\
    && - (J_L^\top X_L^{-1} - J_R^\top X_R^{-1}) \Delta]. \label{eq:torques_with_delta}
\end{IEEEeqnarray}
Now, it is easy to verify that
\begin{align*}
    J_L^\top X_L^{-1} + J_R^\top X_R^{-1} &= \begin{bmatrix}
        2~1_6 \\ \xoverline{J}_{L,j}^\top X_L^{-1} + \xoverline{J}_{R,j}^\top X_R^{-1} - 2 \frac{\xoverline{M}_{bj}^\top}{m}\Lambda^\top
    \end{bmatrix} \\
    J_L^\top X_L^{-1} - J_R^\top X_R^{-1} &= \begin{bmatrix}
        0_{6 \times 6} \\
        \xoverline{J}_{L,j}^\top X_L^{-1} - \xoverline{J}_{R,j}^\top X_R^{-1}
    \end{bmatrix}.
\end{align*}

Observe also that 
\begin{equation*}
    P^\top e_3 = \begin{bmatrix}
        0_{3\times 3} & -S(r) \\
        0_{3\times 3} & \frac{I}{m}-1_3
    \end{bmatrix}e_3 = 0_6 \Rightarrow \Lambda^\top e_3 = 1_6
\end{equation*}
then \eqref{eq:torques_with_delta} becomes 
\begin{IEEEeqnarray}{rCl}
    \label{eq:torques_expression_full}
   \tau &=& - (J_j M_j^{-1})^\dagger J_j M_j^{-1} \left[\right.(\xoverline{J}_{L,j}^\top X_L^{-1} + \xoverline{J}_{R,j}^\top X_R^{-1} \notag\\
    && - 2 \frac{\xoverline{M}_{bj}^\top}{m})\frac{mg}{2}e_3 + (\xoverline{J}_{L,j}^\top X_L^{-1} - \xoverline{J}_{R,j}^\top X_R^{-1})\Delta\left. \right].
\end{IEEEeqnarray}

If we consider the four-bar linkage planar model, we can notice that the number of rows of $J_j$ are greater than the DoFs of the system and thus the product of the first two terms simplifies into the identity matrix. 
As a consequence, the vector $\Delta$ that minimizes the joint torques is given:
\begin{IEEEeqnarray}{rCl}
    \Delta &=& -\frac{mg}{2} \left(\xoverline{J}_{L,j}^\top X_L^{-1}- \xoverline{J}_{R,j}^\top X_R^{-1}\right)^\dagger \notag \\
    && \left(\xoverline{J}_{L,j}^\top X_L^{-1} + \xoverline{J}_{R,j}^\top X_R^{-1}- 2 \frac{\xoverline{M}_{bj}^\top}{m}\right)e_2 \label{eq:delta_torque_min}
\end{IEEEeqnarray}
which, by using the actual expression for the Jacobians, boils down to
\begin{equation}
    \label{eq:delta_simplified_model}
    \Delta = \begin{bmatrix}
        {3 l \cos^2(\xi)}/{10 d \sin(\xi)}\\
        {3l\cos(\xi)}/{10d}\\
        {d}/{4}
    \end{bmatrix}.
\end{equation}

We can now compute the center of pressures $\sigma_L$ and $\sigma_R$.
As before we focus only on the right foot static CoP knowing that the same analysis can be done equally on the other foot.

Taking the forces expression in \eqref{eq:wrenches_feet}, the static CoP of the right foot is
\begin{equation}
    \label{eq:cop_expression}
    \begin{aligned}
        \sigma_R & = \frac{-\frac{1}{2}\rho_1 - \rho_2 \Delta_1 + \rho_1 \Delta_2 - \Delta_3}{\frac{1}{2} - \Delta_2}.
    \end{aligned}    
\end{equation}

\begin{figure}[t]
  \centering
    \includegraphics[width=.9\columnwidth]{imgs/data/simple_mintorques_cop.pdf}
  \caption{Left and right foot CoPs, and CoM during robot motion. The asymptot is in  correspondence of the forces going to zero}
  \label{fig:simple_mintorques_cop}
\end{figure}

By plugging the expression of $\Delta$ we found before we obtain the expression of the static center of pressure as a function of the free variable $\xi$.
Figure~\ref{fig:simple_mintorques_cop} shows its behaviour.

Interestingly, while the solution exhibits more stable CoPs around the centered position, we can notice a divergent behaviour around $\pm 18 [\mathrm{deg}]$.
This is due to the fact that with this solution, the force on one foot goes to zero as the weight is moved towards the other foot.

It is worth noting that in a real application the introduction of inequalities on the CoPs are thus necessary. Figure~\ref{fig:simple_mintorques_qp_cop} shows the effects of choosing $\Delta$ such that the torques are minimized.
As expected the CoP are limited to remain inside the boundaries of the support polygon of the foot.

% Indeed, let's analyze \eqref{eq:cop_expression} by performing an asymptotic analysis.
% \begin{figure}[t]
%   \centering
%     \includegraphics[width=.9\columnwidth]{imgs/data/simple_mintorques_forces.pdf}
%   \caption{Vertical forces for the left and right foot during robot motion for the choice of $\Delta$ as in \eqref{eq:delta_simplified_model}. Forces are normalized by $mg$}
%   \label{fig:simple_mintorques_forces}
% \end{figure}
\begin{figure}[t]
  \centering
    \includegraphics[width=.9\columnwidth]{imgs/data/simple_mintorques_qp_cop.pdf}
  \caption{Left and right foot CoPs, and CoM during robot motion. CoPs remains limited because of the presence of the QP solver}
  \label{fig:simple_mintorques_qp_cop}
\end{figure}
We can compare the static centers of pressure for the two different force solution applied to the system by computing their sensitivity.

We can differentiate the CoP expression w.r.t $\xi$, that is
\begin{align*}
   \eta_R &= \frac{\partial \sigma_R}{\partial \xi} = \frac{\partial}{\partial \xi} \left(\frac{3ld\cos(\xi)}{10d - 6l\cos(\xi)} \right) \\
   & = - \frac{15 l d^2 \sin(\xi)}{2(5d - 3l\cos(\xi))^2}
\end{align*}

\subsection{Static CoP Sensitivity Analysis}

\begin{figure}[t]
  \centering
    \includegraphics[width=.9\columnwidth]{imgs/data/simple_all_cop.pdf}
  \caption{Comparison between the right foot CoPs for two different forces choice. The CoM is also plotted in yellow}
  \label{fig:simple_all_cop}
\end{figure}

We now analyse the sensitivity of the static CoP for the four-bar linkage model when we apply the two different forces solution in \eqref{eq:4bar_minforces} and \eqref{eq:torques_expression_full}.

If we evaluate the sensitivity at the initial configuration, i.e. $\xi = \frac{\pi}{2}$, we obtain that $\eta_R = -0.5941 \mathrm{m/rad}$ for the minimum wrenches norm and $\eta_R = -0.3 \mathrm{m/rad}$ for the minimum torque norm solution.
As it is confirmed by the numerical evaluation in Figure~\ref{fig:simple_all_cop} the second solution is twice less sensitive than the first one.

%
% One issue which becomes apparent when applying the obtained wrenches to the system is related to the centers of pressure.
% % The choice of $\Delta$ in \eqref{eq:delta_torque_min} is in general not good.
% In fact, the CoPs resulting from the forces as in \eqref{eq:wrenches_feet} with $\Delta$ chosen as \eqref{eq:delta_torque_min} tends to infinity.
% This is caused by the fact that while the vertical forces goes to zero, their contact moments does not, thus leading to the observed divergence.
%
% An interesting fact is that this property does not strictly depends on the particular criterion to choose $\Delta$.
%  % but it is instead related to how  re on the fact that the force goes to zero on the non-support foot and on how its moment is chosen.
% To show this fact we can perform an asymptotical analysis on the center of pressure.
%
% Let's recall the definition of the center of pressure, which for the considered 2D case corresponds to a single coordinate along $e_1$:
% \begin{equation*}
%     CoP = \frac{\mu}{f_{e_2}},
% \end{equation*}
% which become for two feet:
% \begin{equation}
%     \label{eq:cop_expression}
%     \begin{aligned}
%         CoP_L &= \frac{\mu_L}{f_{L_{ne_2}}} = \frac{-\frac{1}{2}\lambda_1 + \lambda_2 \Delta_1 - \lambda_1 \Delta_2 + \Delta_3}{\frac{1}{2} + \Delta_2} \\
%         CoP_R &= \frac{\mu_R}{f_{R_{e_2}}} = \frac{-\frac{1}{2}\rho_1 - \rho_2 \Delta_1 + \rho_1 \Delta_2 - \Delta_3}{\frac{1}{2} - \Delta_2}.
%     \end{aligned}
% \end{equation}
%
% We now focus on the case where the center of mass is on the right foot, i.e. the right foot supports the whole weight. The same consideration can be done equally for the other foot.
% Because of this, $f_{R_{e_2}} = mg$, which, as a consequence of \eqref{eq:solution_explicit}, implies $\Delta_2 = -\frac{1}{2}$.
% The CoP of the left foot thus become
% \begin{align*}
%     CoP_L &= \lim_{\Delta_2 \rightarrow -\frac{1}{2}} \frac{-\frac{1}{2}\lambda_1 + \lambda_2 \Delta_1 - \lambda_1 \Delta_2 + \Delta_3}{\frac{1}{2} + \Delta_2} \\
%     &= \frac{\lambda_2 \Delta_1 + \Delta_3}{0}.
% \end{align*}
%
% The result of the above expression depends on the value of the numerator, i.e. of $\lambda_2 \Delta_1 + \Delta_3$.
% Indeed, if it is different from zero, then the CoP tends to $\pm \infty$.
% If, instead, it goes to zero faster then the denominator, the CoP tends to zero.
%
% If we consider the expression of $\Delta$ in \eqref{eq:delta_simplified_model} we can verify that the CoP diverges.
% In fact
% \begin{align*}
%     &\Delta_2 = -\frac{1}{2} \Rightarrow \cos(q_1) = - \frac{5d}{3l} \\
%     &\Rightarrow \Delta_1 = \frac{5d}{6l\sin(q_1)}, \quad \Delta_3 = \frac{d}{4}.
% \end{align*}
% Furthermore $\lambda_2$ has the following expression:
% \begin{equation*}
%     \lambda_2 = %\frac{2m_B + m_L + m_R}{m_B + m_L + m_R} \frac{l}{4} \sin(q_1)
%      -\alpha \frac{l}{2} \sin(q_1)
% \end{equation*}
% where $\alpha > 1$ is a term which depends on the mass of the three rods. By plugging everything together we get:
% \begin{align*}
%     \lambda_2 \Delta_1 + \Delta_3 &= -\alpha \frac{l}{2} \sin(q_1)  \frac{5d}{6l\sin(q_1)} + \frac{d}{4} = \frac{d(3 - 5 \alpha)}{12} < 0.
% \end{align*}
% Given the above result $CoP_L \rightarrow - \infty$.
%
%
%
% Figure~\ref{fig:simple_mintorques_cop} shows the CoPs during the robot motion. Notice that the CoP of the left foot goes to $-\infty$ when the left force in Figure~\ref{fig:simple_mintorques_forces} goes to zero, as expected.
%
% It is interesting to compare the obtained CoPs and wrenches with the results from Remark~\ref{lemma:cop_forces}.
% The hypothesis of the statement in this case are not satisfied.
% When the center of mass is on top of one CoP, the two CoP coincides, i.e. $\lambda_{cop_1} - \rho_{cop_1} = 0$.
% % If we consider the point where the vertical force goes to zero, then it is the CoPs which goes to infinity.
%
% Different solutions can be put into effect in order to satisfy Remark~\ref{lemma:cop_forces} and thus having limited CoPs while forces go to zero.
% One possible way is to find a new optimization criterion to exploit the forces redundancy.
% Alternatively, one can try to impose conditions on the first and third components of $\Delta$ in \eqref{eq:cop_expression}.
% Indeed, trying to impose that the numerator goes to zero faster than the denominator can result in a nonlinear problem.
%
% A pragmatic approach, instead, is to use a QP solver to include inequalities on the CoPs. Note that in a real world application, inequalities are anyways needed to satisfy friction cones, joint torque limits, and other constraints.
%
% \begin{figure}[t]
%   \centering
%     \includegraphics[width=.9\columnwidth]{imgs/data/simple_mintorques_qp_cop.pdf}
%   \caption{Left and right foot CoPs, and CoM during robot motion. CoPs remains limited because of the presence of the QP solver}
%   \label{fig:simple_mintorques_qp_cop}
% \end{figure}
%
% If we solve \eqref{eq:torques_expression_full} by using a dedicated solver we obtain the CoPs as in Figure~\ref{fig:simple_mintorques_qp_cop}.
% Forces are not shown because they are similar to the ones in Figure~\ref{fig:simple_mintorques_forces}.
% We can note that in this case the center of mass is on top of the center of pressure when the force goes to zero, both for the left foot and for the right foot. The hypotesis of Remark~\ref{lemma:cop_forces} are indeed satisfied.
%
% \subsection{Static CoP Sensitivity Analysis}
%
% We now analyse the sensitivity of the static CoP for the four-bar linkage model when we apply the two different forces solution in \eqref{} and \eqref{eq:torques_expression_full}.
% We show the analysis we performed on the right foot, but the same results can be drawn for the left foot.
%
% If we denote with $q$ the minimum coordinate of the constrained four-bar linkage model we can differentiate the CoP expression, that is
% \begin{align*}
%     \frac{\partial CoP_R}{\partial q} &= \frac{\partial}{\partial q} \left(\frac{12 l \cos(q)}{5 d^2 - 6 l d \cos(q) + 20}\right) \\
%     & = -60 l \sin(q) \frac{d^2 + 4}{(5 d^2 - 6 l d \cos(q) + 20)^2}
% \end{align*}
%
% If, instead, we use the forces in \eqref{} we obtain the following expression for the static CoP sensitivity
% \begin{align*}
%    \frac{\partial CoP_R}{\partial q} &= \frac{\partial}{\partial q} \left(\frac{3ld\cos(q)}{10d - 6l\cos(q)} \right) \\
%    & = - \frac{15 l d^2 \sin(q)}{2(5d - 3l\cos(q))^2}
% \end{align*}
%
% \begin{figure}[t]
%   \centering
%     \includegraphics[width=.9\columnwidth]{imgs/data/simple_all_cop.pdf}
%   \caption{Comparison between the right foot CoPs for two different forces choice. The CoM is also plotted in yellow}
%   \label{fig:simple_all_cop}
% \end{figure}
%
% Figure \ref{fig:simple_all_cop} shows the numerical simulations of the CoP of the right foot.
% If we compute the sensitivity at the initial configuration, i.e. $q = \frac{\pi}{2}$, and we use $d = 0.2 \mathrm{m}$ and $l = 1 \mathrm{m}$ we obtain the following values for the two solutions: $-0.5941 \mathrm{m/rad}$ and $-0.3 \mathrm{m/rad}$, i.e. the minimum torque solution is twice less sensitive than the minimum force norm solution.
%
%
%
%
%
%
%
%
%
%
%
%
% Because the matrix
%
% Let's consider the model introduced in the previous section where we have only two external wrenches $f_L$ and $f_R$ resulting from the contact of the robot legs and the ground.
% Being a quasi-static scenario, the sum of the external wrenches and the wrench due to gravity must balance, i.e.
% \begin{align}
%     &W_L + W_R - mg e_2 = 0 \label{eq:momentum_balance} \\
%     &W_L = X_L  \prescript{L}{}f_L,\quad  W_R = X_R \prescript{R}{}f_R \notag\\
%     & X_L = \begin{bmatrix}
%         1_2 & 0_{2\times1} \\ (S\lambda)^\top & 1
%     \end{bmatrix},
%     X_R = \begin{bmatrix}
%         1_2 & 0_{2\times1} \\ (S\rho)^\top & 1
%     \end{bmatrix} \notag
% \end{align}
% where $\lambda$ and $\rho$ are the vectors from the center of mass to the left and right contacts respectively and the left and right wrenches $f_L = \begin{bmatrix}F_L^\top & \mu_L\end{bmatrix}^\top$, $f_R = \begin{bmatrix}F_R^\top & \mu_R\end{bmatrix}^\top$ are composed by the pure forces and pure torques.
%
% Now, we can impose the following form for the contact wrenches:
% \begin{equation}
%     \label{eq:wrench_decomposition}
%     \begin{aligned}
%         W_L &= W_m + \Delta \\
%         W_R &= W_m - \Delta
%     \end{aligned}
% \end{equation}
% The above definition must satisfy \eqref{eq:momentum_balance}. We thus get
% \begin{align*}
%     W_m &= \frac{W_L + W_R}{2} = \frac{mg}{2}e_2\\
%     \Delta &\in \mathbb{R}^3 \quad \text{free} .% \frac{W_L - W_R}{2}\\
% \end{align*}
% The wrenches expressed at the feet now becomes
% \begin{equation}
%     \label{eq:wrenches_feet}
%     \begin{aligned}
%         \prescript{L}{} f_L &= X_L^{-1} W_m + X_L^{-1} \Delta \\
%         \prescript{R}{} f_R &= X_R^{-1} W_m - X_R^{-1} \Delta \\
%     \end{aligned}
% \end{equation}
% By substituting the definition of $W_m$, $X_L$ and of $X_R$ we obtain the following expression:
% \begin{equation}
%     \label{eq:solution_explicit}
%     \begin{aligned}
%         \prescript{L}{}f_L &= \frac{mg}{2}\begin{bmatrix}
%             0 \\ 1 \\ -\lambda_1
%         \end{bmatrix} + X_L^{-1} \Delta \\
%         \prescript{R}{}f_R &= \frac{mg}{2}\begin{bmatrix}
%             0 \\ 1 \\ -\rho_1
%         \end{bmatrix} - X_R^{-1} \Delta
%     \end{aligned}
% \end{equation}
%
% Because $\Delta$ is a free variable one may be tempted to choose the trivial solution, i.e. $\Delta = 0$.
% This choice leads to constant vertical (and equal) forces on both feet, i.e. $(\prescript{L}{}{f_L})_2 = ({\prescript{R}{}{f_R}})_2 = \frac{mg}{2}$.
% They are thus independent of the CoM position.
% What, instead, varies with the CoM position are the contact torques which have to compensate for this internal stress.
%
% Notice that the solution obtained with $\Delta = 0$ is similar to the minimum norm solution to \eqref{eq:momentum_balance}.
% In fact,
% \begin{align*}
%     mg e_2 &= W_L + W_R =
%     \begin{bmatrix}
%         X_L & X_R
%     \end{bmatrix} \begin{bmatrix}
%         \prescript{L}{}f_L \\ \prescript{R}{}f_R
%     \end{bmatrix} = X f
% \end{align*}
%
% Because, by construction, $X$ is always full row rank we can use the explicit expression of its pseudoinverse to obtain an analytical solution for the wrenches $f$.
% In particular, we are interested in the difference between the linear components $\Delta F = F_L - F_R$ which has the following expression:
% \begin{equation}
%     \label{eq:minimum_norm_solution}
%     \begin{aligned}
%         \Delta F &= \frac{mg}{4 + \norm{\lambda - \rho}^2} S(\lambda - \rho)(\lambda + \rho)^\top S e_2 \\
%         &= - \frac{mg (\lambda_1 - \rho_1)^2}{4 + (\lambda_1 - \rho_1)^2}e_2
%     \end{aligned}
% \end{equation}
% where we used the fact that $\lambda - \rho$ is zero along the $e_2$ axis.
%
% The above equation clearly points out two properties of the solution.
% The first one is that the difference lies only in the vertical component ($e_2$).
% The second one is that this difference is function of the distance between the two feet (constant in our scenario), and it is not a function of the CoM position.
%
% This fact is compatible with the analysis performed on the full model of the robot we showed in Section~\ref{sec:background}.
% The minimum norm solution of \eqref{eq:momentum_balance} has thus similar effects of the solution \eqref{eq:solution_explicit} with $\Delta = 0$.
%
% % Both the solutions previously obtained may seem counterintuitive, especially while comparing them to what humans do.
% % Indeed, one may expect that the force not on the support foot tends to zero as the center of mass moves towards  the support foot.
% We now try to find if a different feasible choice of the contact forces leads to a different behaviour.
% Let's first consider again \eqref{eq:momentum_balance} but with the forces expressed at the local center of pressure (CoP) instead of the origin of the foot frames.
% As a consequence the pure torques are zeros, i.e. \eqref{eq:momentum_balance} rewrites as
% \begin{equation*}
%     \label{eq:momentum_balance_cop}
%     \begin{aligned}
%          F_L + F_R & = mg e_2 \\
%          \lambda_{cop}^\top S F_L + \rho_{cop}^\top S F_R &= 0
%     \end{aligned}
% \end{equation*}
% where $\lambda_{cop}$ and $\rho_{cop}$ are the vectors connecting the CoM to the center of pressure of the left and right foot respectively.
% Analogously to \eqref{eq:wrench_decomposition} we can decompose the forces as
% \begin{equation}
%     \label{eq:wrench_decomposition_cop}
%     \begin{aligned}
%         F_L &= F_m + \tilde{\Delta}\\
%         F_R &= F_m - \tilde{\Delta}\\
%     \end{aligned}
% \end{equation}
% where now $\tilde{\Delta} \in \mathbb{R}^2$. By imposing \eqref{eq:momentum_balance_cop}, one obtains
% \begin{equation*}
%     \begin{aligned}
%         F_m &= \frac{mg}{2} e_2 \\
%         \tilde{\Delta} &= - \frac{(\lambda_{cop}+\rho_{cop})^\top e_1}{(\lambda_{cop}-\rho_{cop})^\top e_1} \frac{mg}{2}e_2 + \eta e_1
%     \end{aligned}
% \end{equation*}
% with $\eta \in \mathbb{R}$ free.
% By substituting the definition of $F_m$ and of $\tilde{\Delta}$ into \eqref{eq:wrench_decomposition_cop} we obtain the final expression for the feet forces:
% \begin{equation}
%     \label{eq:solution_explicit_cop}
%     \begin{aligned}
%         F_L &= - \frac{\rho_{cop_1}}{\lambda_{cop_1} - \rho_{cop_1}}mge_2 + \eta e_1 \\
%         F_R &=  \frac{\lambda_{cop_1}}{\lambda_{cop_1} - \rho_{cop_1}}mge_2 + \eta e_1
%     \end{aligned}
% \end{equation}
%
% We can now do the following statement:
% \begin{Remark} \label{lemma:cop_forces}
%     If $\lambda_{cop_1} \neq \rho_{cop_1} \iff CoP_L \neq CoP_R$ (written w.r.t the world frame) and $\lambda_{cop_1} - \rho_{cop_1}$ is finite, then the vertical right (left) force is equal to zero when the center of mass is above the left (right) center of pressure.
% \end{Remark}
% \begin{proof}
% The proof comes from the application of \eqref{eq:solution_explicit_cop}.
% In fact if the CoM is above the left foot, then by definition $\lambda_{cop_1} = 0$. Given \eqref{eq:solution_explicit_cop} and the fact that the denominator is finite by hypothesis then $F_R = 0$. The same reasoning can be applied to the right foot.
% The first hypotesis of this remark guarantees that at least one foot must support the weight of the robot.
% \end{proof}
%
% \subsection{Choice of the force redundancy}
% The analysis conducted in the previous section and the results in Remark~\ref{lemma:cop_forces} shows that the choice of contact forces is responsible of different behaviours in the robot.
% A part from the motivations already introduced in Section~\ref{subsec:problem_statement}, forces as in \eqref{eq:solution_explicit_cop} avoid creating internal stress.
% We now wonder if there exist a criterion to systematically exploit the redundancy of the forces in \eqref{eq:solution_explicit}, i.e. a choice of the variable $\Delta$, to obtain a behaviour similar to the one stated in Remark~\ref{lemma:cop_forces}.
%
% Because internal stress in the structure is due to internal torques compensating each other, one possible criterion for the choice of $\Delta$ is to use the redundancy to minimize the internal joint torques.
% Let's notice however that in case of a mechanical system with heterogeneous joint types, e.g. rotational and prismatic joints, the euclidean norm of the generalized forces is not well defined.
% This criterion is anyway justifiable by remembering that the torque produced by an electric motor is proportional to the current absorption and thus to the electric power. Similar considerations can be done for other types of motors.
%
% Assuming rotational joints for simplicity, let's consider \eqref{eq:tau_block_diagonal} and use the wrenches expression in \eqref{eq:wrenches_feet}:
% \begin{IEEEeqnarray}{rCl}
%     \tau &=& (J_j M_j^{-1})^\dagger J M^{-1} (mge_3 - J_L^\top f_L - J_R^\top f_R) \notag\\
%     &=& (J_j M_j^{-1})^\dagger J M^{-1} [ (2 - J_L^\top X_L^{-1} - J_R^\top X_R^{-1}) \frac{mg}{2}e_3 \notag\\
%     && - (J_L^\top X_L^{-1} - J_R^\top X_R^{-1}) \Delta] \label{eq:torques_with_delta}
% \end{IEEEeqnarray}
%
% By using the definition of the Jacobian of a generic point $p$ as in \eqref{eq:block_diag_relations}
% % Recalling the definition of the Jacobian of a generic point $p$ in the dynamical model \eqref{eq:system_dynamics}
% % \begin{equation*}
% %     J_p^\top =
% %     \begin{bmatrix}
% %         X_p \\
% %         \xoverline{J}^\top_{p,j} - \frac{\xoverline{M}_{bj}^\top}{m} \Lambda^\top X_p
% %     \end{bmatrix}
% % \end{equation*}
% we obtain:
% \begin{align*}
%     J_L^\top X_L^{-1} + J_R^\top X_R^{-1} &= \begin{bmatrix}
%         2~1_6 \\ \xoverline{J}_{L,j}^\top X_L^{-1} + \xoverline{J}_{R,j}^\top X_R^{-1} - 2 \frac{\xoverline{M}_{bj}^\top}{m}\Lambda^\top
%     \end{bmatrix} \\
%     J_L^\top X_L^{-1} - J_R^\top X_R^{-1} &= \begin{bmatrix}
%         0_{6 \times 6} \\
%         \xoverline{J}_{L,j}^\top X_L^{-1} - \xoverline{J}_{R,j}^\top X_R^{-1}
%     \end{bmatrix}.
% \end{align*}
%
% Observe also that
% \begin{equation*}
%     P^\top e_3 = \begin{bmatrix}
%         0_{3\times 3} & -S(r) \\
%         0_{3\times 3} & \frac{I}{m}-1_3
%     \end{bmatrix}e_3 = 0_6 \Rightarrow \Lambda^\top e_3 = 1_6
% \end{equation*}
% then \eqref{eq:torques_with_delta} becomes
% \begin{IEEEeqnarray}{rCl}
%     \label{eq:torques_expression_full}
%     % \tau &=& (J_j M_j^{-1})^\dagger J \begin{bmatrix} M_b^{-1} & 0 \\ 0 & M_j^{-1} \end{bmatrix}\notag\\
%  %    && \left( \right.
%  %    \begin{bmatrix}mge_2 - mge_2  \\
%  %        -(\xoverline{J}_{jL}^\top X_L^{-1} + \xoverline{J}_{jR}^\top X_R^{-1} - 2 \frac{\xoverline{M}_{bj}^\top}{m})\frac{mg}{2}e_2
%  %    \end{bmatrix} \notag\\
%  %    &&- \begin{bmatrix}
%  %        0_3 \\ \xoverline{J}_{jL}^\top X_L^{-1} - \xoverline{J}_{jR}^\top X_R^{-1}
%  %    \end{bmatrix} \Delta \left. \right) \notag\\
%    \tau &=& - (J_j M_j^{-1})^\dagger J_j M_j^{-1} \left[\right.(\xoverline{J}_{L,j}^\top X_L^{-1} + \xoverline{J}_{R,j}^\top X_R^{-1} \notag\\
%     && - 2 \frac{\xoverline{M}_{bj}^\top}{m})\frac{mg}{2}e_3 + (\xoverline{J}_{L,j}^\top X_L^{-1} - \xoverline{J}_{R,j}^\top X_R^{-1})\Delta\left. \right].
% \end{IEEEeqnarray}
%
% When we consider the simplified model, we can notice that if the number of (nonsingular) rows of $J_j$ are greater or equal to the DoFs of the system, as it is in this case, the product of the first two terms yield the identity matrix.
% As a consequence, the vector $\Delta$ which minimizes the joint torques in the four-bar linkage model is given by the solution of
% \begin{IEEEeqnarray}{rCl}
%     \Delta &=& -\frac{mg}{2} \left(\xoverline{J}_{L,j}^\top X_L^{-1}- \xoverline{J}_{R,j}^\top X_R^{-1}\right)^\dagger \notag \\
%     && \left(\xoverline{J}_{L,j}^\top X_L^{-1} + \xoverline{J}_{R,j}^\top X_R^{-1}- 2 \frac{\xoverline{M}_{bj}^\top}{m}\right)e_2 \label{eq:delta_torque_min}
% \end{IEEEeqnarray}
% which, by using the actual expression for the Jacobians, can be simplified to
% \begin{equation}
%     \label{eq:delta_simplified_model}
%     \Delta = \begin{bmatrix}
%         {3 l \cos^2(q_1)}/{10 d \sin(q_1)}\\
%         {3l\cos(q_1)}/{10d}\\
%         {d}/{4}
%     \end{bmatrix}.
% \end{equation}
%
% Interestingly, the linear forces are function of $\frac{l}{d}$, i.e. the ratio between the length of the legs and the feet distance. Furthermore, as we expected, they are also function of the angle $q_1$ thus varying with the configuration of the robot.
% Figure~\ref{fig:simple_mintorques_forces} shows the vertical forces for the two feet when the choice of $\Delta$ is the one in \eqref{eq:delta_simplified_model}.
%
% \begin{figure}[t]
%   \centering
%     \includegraphics[width=.9\columnwidth]{imgs/data/simple_mintorques_forces.pdf}
%   \caption{Vertical forces for the left and right foot during robot motion for the choice of $\Delta$ as in \eqref{eq:delta_simplified_model}. Forces are normalized by $mg$}
%   \label{fig:simple_mintorques_forces}
% \end{figure}
%
% \subsection{Analysis of the centers of pressure}
% One issue which becomes apparent when applying the obtained wrenches to the system is related to the centers of pressure.
% % The choice of $\Delta$ in \eqref{eq:delta_torque_min} is in general not good.
% In fact, the CoPs resulting from the forces as in \eqref{eq:wrenches_feet} with $\Delta$ chosen as \eqref{eq:delta_torque_min} tends to infinity.
% This is caused by the fact that while the vertical forces goes to zero, their contact moments does not, thus leading to the observed divergence.
%
% An interesting fact is that this property does not strictly depends on the particular criterion to choose $\Delta$.
%  % but it is instead related to how  re on the fact that the force goes to zero on the non-support foot and on how its moment is chosen.
% To show this fact we can perform an asymptotical analysis on the center of pressure.
%
% Let's recall the definition of the center of pressure, which for the considered 2D case corresponds to a single coordinate along $e_1$:
% \begin{equation*}
%     CoP = \frac{\mu}{f_{e_2}},
% \end{equation*}
% which become for two feet:
% \begin{equation}
%     \label{eq:cop_expression}
%     \begin{aligned}
%         CoP_L &= \frac{\mu_L}{f_{L_{e_2}}} = \frac{-\frac{1}{2}\lambda_1 + \lambda_2 \Delta_1 - \lambda_1 \Delta_2 + \Delta_3}{\frac{1}{2} + \Delta_2} \\
%         CoP_R &= \frac{\mu_R}{f_{R_{e_2}}} = \frac{-\frac{1}{2}\rho_1 - \rho_2 \Delta_1 + \rho_1 \Delta_2 - \Delta_3}{\frac{1}{2} - \Delta_2}.
%     \end{aligned}
% \end{equation}
%
% We now focus on the case where the center of mass is on the right foot, i.e. the right foot supports the whole weight. The same consideration can be done equally for the other foot.
% Because of this, $f_{R_{e_2}} = mg$, which, as a consequence of \eqref{eq:solution_explicit}, implies $\Delta_2 = -\frac{1}{2}$.
% The CoP of the left foot thus become
% \begin{align*}
%     CoP_L &= \lim_{\Delta_2 \rightarrow -\frac{1}{2}} \frac{-\frac{1}{2}\lambda_1 + \lambda_2 \Delta_1 - \lambda_1 \Delta_2 + \Delta_3}{\frac{1}{2} + \Delta_2} \\
%     &= \frac{\lambda_2 \Delta_1 + \Delta_3}{0}.
% \end{align*}
%
% The result of the above expression depends on the value of the numerator, i.e. of $\lambda_2 \Delta_1 + \Delta_3$.
% Indeed, if it is different from zero, then the CoP tends to $\pm \infty$.
% If, instead, it goes to zero faster then the denominator, the CoP tends to zero.
%
% If we consider the expression of $\Delta$ in \eqref{eq:delta_simplified_model} we can verify that the CoP diverges.
% In fact
% \begin{align*}
%     &\Delta_2 = -\frac{1}{2} \Rightarrow \cos(q_1) = - \frac{5d}{3l} \\
%     &\Rightarrow \Delta_1 = \frac{5d}{6l\sin(q_1)}, \quad \Delta_3 = \frac{d}{4}.
% \end{align*}
% Furthermore $\lambda_2$ has the following expression:
% \begin{equation*}
%     \lambda_2 = %\frac{2m_B + m_L + m_R}{m_B + m_L + m_R} \frac{l}{4} \sin(q_1)
%      -\alpha \frac{l}{2} \sin(q_1)
% \end{equation*}
% where $\alpha > 1$ is a term which depends on the mass of the three rods. By plugging everything together we get:
% \begin{align*}
%     \lambda_2 \Delta_1 + \Delta_3 &= -\alpha \frac{l}{2} \sin(q_1)  \frac{5d}{6l\sin(q_1)} + \frac{d}{4} = \frac{d(3 - 5 \alpha)}{12} < 0.
% \end{align*}
% Given the above result $CoP_L \rightarrow - \infty$.
%
% \begin{figure}[t]
%   \centering
%     \includegraphics[width=.9\columnwidth]{imgs/data/simple_mintorques_cop.pdf}
%   \caption{Left and right foot CoPs, and CoM during robot motion. The asymptot is in  correspondence of the forces going to zero}
%   \label{fig:simple_mintorques_cop}
% \end{figure}
%
% Figure~\ref{fig:simple_mintorques_cop} shows the CoPs during the robot motion. Notice that the CoP of the left foot goes to $-\infty$ when the left force in Figure~\ref{fig:simple_mintorques_forces} goes to zero, as expected.
%
% It is interesting to compare the obtained CoPs and wrenches with the results from Remark~\ref{lemma:cop_forces}.
% The hypothesis of the statement in this case are not satisfied.
% When the center of mass is on top of one CoP, the two CoP coincides, i.e. $\lambda_{cop_1} - \rho_{cop_1} = 0$.
% % If we consider the point where the vertical force goes to zero, then it is the CoPs which goes to infinity.
%
% Different solutions can be put into effect in order to satisfy Remark~\ref{lemma:cop_forces} and thus having limited CoPs while forces go to zero.
% One possible way is to find a new optimization criterion to exploit the forces redundancy.
% Alternatively, one can try to impose conditions on the first and third components of $\Delta$ in \eqref{eq:cop_expression}.
% Indeed, trying to impose that the numerator goes to zero faster than the denominator can result in a nonlinear problem.
%
% A pragmatic approach, instead, is to use a QP solver to include inequalities on the CoPs. Note that in a real world application, inequalities are anyways needed to satisfy friction cones, joint torque limits, and other constraints.
%
% \begin{figure}[t]
%   \centering
%     \includegraphics[width=.9\columnwidth]{imgs/data/simple_mintorques_qp_cop.pdf}
%   \caption{Left and right foot CoPs, and CoM during robot motion. CoPs remains limited because of the presence of the QP solver}
%   \label{fig:simple_mintorques_qp_cop}
% \end{figure}
%
% If we solve \eqref{eq:torques_expression_full} by using a dedicated solver we obtain the CoPs as in Figure~\ref{fig:simple_mintorques_qp_cop}.
% Forces are not shown because they are similar to the ones in Figure~\ref{fig:simple_mintorques_forces}.
% We can note that in this case the center of mass is on top of the center of pressure when the force goes to zero, both for the left foot and for the right foot. The hypotesis of Remark~\ref{lemma:cop_forces} are indeed satisfied.
%
% \subsection{Static CoP Sensitivity Analysis}
%
% We now analyse the sensitivity of the static CoP for the four-bar linkage model when we apply the two different forces solution in \eqref{} and \eqref{eq:torques_expression_full}.
% We show the analysis we performed on the right foot, but the same results can be drawn for the left foot.
%
% If we denote with $q$ the minimum coordinate of the constrained four-bar linkage model we can differentiate the CoP expression, that is
% \begin{align*}
%     \frac{\partial CoP_R}{\partial q} &= \frac{\partial}{\partial q} \left(\frac{12 l \cos(q)}{5 d^2 - 6 l d \cos(q) + 20}\right) \\
%     & = -60 l \sin(q) \frac{d^2 + 4}{(5 d^2 - 6 l d \cos(q) + 20)^2}
% \end{align*}
%
% If, instead, we use the forces in \eqref{} we obtain the following expression for the static CoP sensitivity
% \begin{align*}
%    \frac{\partial CoP_R}{\partial q} &= \frac{\partial}{\partial q} \left(\frac{3ld\cos(q)}{10d - 6l\cos(q)} \right) \\
%    & = - \frac{15 l d^2 \sin(q)}{2(5d - 3l\cos(q))^2}
% \end{align*}
%
% \begin{figure}[t]
%   \centering
%     \includegraphics[width=.9\columnwidth]{imgs/data/simple_all_cop.pdf}
%   \caption{Comparison between the right foot CoPs for two different forces choice. The CoM is also plotted in yellow}
%   \label{fig:simple_all_cop}
% \end{figure}
%
% Figure \ref{fig:simple_all_cop} shows the numerical simulations of the CoP of the right foot.
% If we compute the sensitivity at the initial configuration, i.e. $q = \frac{\pi}{2}$, and we use $d = 0.2 \mathrm{m}$ and $l = 1 \mathrm{m}$ we obtain the following values for the two solutions: $-0.5941 \mathrm{m/rad}$ and $-0.3 \mathrm{m/rad}$, i.e. the minimum torque solution is twice less sensitive than the minimum force norm solution.
%
%


==> tex/modelling.tex <==
%!TEX root = ../tau_optim.tex
\section{Modelling}
\label{sec:modelling}
\subsection{Block Diagonalization of the Mass Matrix}
The dynamics in \eqref{eq:system_dynamics} in written with no assumptions on the location of the base frame, a part being rigidly connected to the system.

If we assume that the Pl\"ucker frame of the base is written with the orientation coinciding with the inertial frame and the origin to be placed instantaneously on the center of mass, the resulting dynamic equation exhibits a block diagonal mass matrix, that is
\begin{equation*}
    M(q) = \begin{bmatrix}
        M_b(q) & 0 \\ 0 & M_j(q)
    \end{bmatrix}
\end{equation*}
where $M_b \in \mathbb{R}^{6 \times 6}$ is the base term and $M_j \in \mathbb{R}^{n \times n}$ is the joint term.

If we further assume that the first $6$ rows are written w.r.t. a frame with the origin located in the center of mass then the mass matrix of the base term can be further simplified as:
\begin{equation*}
    M_b(q) = \begin{bmatrix}
        m 1_3 & 0 \\ 0 & I(q)
    \end{bmatrix}
\end{equation*}
where $m$ is the mass of the robot and $I$ is the inertia matrix.

Note that these assumptions are not limiting. 
Indeed, it is always possible to transform the system into the block-diagonal form by means of a change of basis.

Let's denote with the bar, $\xoverline{(\cdot)}$, the elements of the non block-diagonal dynamic equation \eqref{eq:system_dynamics}, i.e. the following equation
\begin{align*}
    \xoverline{M}(q)\dot{\xoverline{\nu}} + \xoverline{C}(q, \xoverline{\nu})\xoverline{\nu} + \xoverline{g}(q) = D \tau + \xoverline{J}^\top(q) f
\end{align*}
has not the mass matrix in block diagonal form.
Indeed, the mass matrix has the following generic form:
\begin{equation*}
    \xoverline{M} = \begin{bmatrix}
        \xoverline{M}_b & \xoverline{M}_{bj} \\
        \xoverline{M}_{bj}^\top & \xoverline{M}_j
    \end{bmatrix} .
\end{equation*}

Let's perform the following change of basis $\nu = T \xoverline{\nu}$, with 
\begin{align*}
    T &:= \begin{bmatrix}
        \prescript{c}{}X_{b} & T_s \\
        0_{n \times 6} & 1_n
    \end{bmatrix}, T_s = \prescript{c}{}X_{b} \xoverline{M}^{-1}_b \xoverline{M}_{bj} \\
    \prescript{c}{}X_{b} &:= \begin{bmatrix}
        1_3 & -S(r) \\ 
        0_{3 \times 3} & 1_3
    \end{bmatrix}
\end{align*}
where $r = c - b$ is the vector going from the origin of the base to the center of mass and $\prescript{c}{}X_{b}$ is the trasformation matrix from the base frame to the frame centered in the center of mass, with the orientation written w.r.t. the inertial frame.

Applying the change of basis we obtain the dynamics written as in \eqref{eq:system_dynamics} with the following relations:
\begin{equation}
    \label{eq:block_diag_relations}
    \begin{aligned}
        M &= T^{-\top} \xoverline{M} T^{-1}, C = T^{-\top}(\xoverline{M}\dot{T}^{-1} + \xoverline{C}T^{-1}) \\
        g &= T^{-\top}\xoverline{g} = mg e_3 \\
        J_p &= \xoverline{J}_pT^{-1} = \begin{bmatrix}
            X_p^\top & {\xoverline{J}_{p,j}} - \frac{X_p^\top}{m} \Lambda \xoverline{M}_{bj}
        \end{bmatrix} \\
        \Lambda &= 1_6 - P (1_6 + \prescript{c}{}X_b^{-1} P)^{-1} \prescript{c}{}X_b^{-1} \\
        X_p &= \begin{bmatrix}
            1_3 & 0_{3 \times 3} \\
            S (r_p) & 1_3
        \end{bmatrix}, P = \begin{bmatrix}
            0_{3\times 3} & 0_{3\times 3} \\ S(r) & \frac{I}{m} - 1_3
        \end{bmatrix}
    \end{aligned}
\end{equation}
where $r_p = c - p$ is the vector going from the CoM to the force application point $p$.

If we now assume that the dynamical system \eqref{eq:system_dynamics} is written with the block diagonal mass matrix, we can rewrite the control torques in \eqref{eq:tau_generic} as:
\begin{align}
    \label{eq:tau_block_diagonal}
    \tau &= (J_j M_j^{-1})^\dagger[JM^{-1}(C \nu + mg e_3 - J^\top f) - \dot{J}\nu] + N_\tau \tau_0.
\end{align}


\subsection{Simplified Model}

\begin{figure}
    \centering{
    % \includsvg{imgs/model}
        \def\svgwidth{\columnwidth}
        \input{imgs/model.pdf_tex}
    \caption{Simplified model: planar four-bar linkage}
    \label{fig:simple_model}
    }
\end{figure}

The analysis that we present in the next section will be conducted mainly on a simplified model and not on the full dynamical model \eqref{eq:system_dynamics}.

As we can observe in Figure~\ref{fig:simple_model} we consider a planar four-bar linkage. The system has thus four degrees of freedom. The base frame is located in the center of the upper connecting rod.
The length of the ``leg'' rods is $l$, while the upper rod length is $d$. 

Being in a two dimensional space, we allow only translations on the $y$ and $z$ axes, and rotation along the $x$ axis.
The configuration variable $q \in (\mathbb{R}^2 \times S^1) \times \mathbb{R}^4$ and $\nu \in \mathbb{R}^{7}$.

We assume the feet do not move and remains at the same distance of the upper rod, i.e. $d$, thus in the centered position all the angles are equal to $\frac{\pi}{2}$ and the legs are parallel.
We will also consider quasi-static scenarios, i.e. the velocity is zero.



